Fast Complementary Dynamics via Skinning Eigenmodes

We propose a reduced-space elasto-dynamic solver that is well suited for augmenting rigged character animations with secondary motion. At the core of our method is a novel deformation subspace based on Linear Blend Skinning that overcomes many of the shortcomings prior subspace methods face. Our skinning subspace is parameterized entirely by a set of scalar weights, which we can obtain through a small, material-aware and rig-sensitive generalized eigenvalue problem. The resulting subspace can easily capture rotational motion and guarantees that the resulting simulation is rotation equivariant. We further propose a simple local-global solver for linear co-rotational elasticity and propose a clustering method to aggregate per-tetrahedra non-linear energetic quantities. The result is a compact simulation that is fully decoupled from the complexity of the mesh.

==> localized_modes.tex <==
\subsubsection{Localized Modes}
Given a locality length scale $r$ and a center of locality $\boldsymbol{c}_i$, we aim to find a set of modes that are entirely located within a specific region of the mesh $\boldsymbol{S}^T (\boldsymbol{c}_i; r) \boldsymbol{b}_i= \boldsymbol{0}$, where $\boldsymbol{S} \in \mathbb{R}^{n \times m}$ is a selection matrix that selects the m-vertices that are \emph{not} within our region of locality.

We treat the locality length scale $r$ as an input user parameter, and the centers of locality as degrees of freedom in our GEVP energy minimization. Enforcing the constraint above into our GEVP:

\begin{align}
\argmin_{\boldsymbol{b}_i, \boldsymbol{c}_i}\,&  \boldsymbol{b}_i^T \boldsymbol{H} \boldsymbol{b}_i \\  \text{s.t.} \quad \boldsymbol{S}(\boldsymbol{c}_i; \boldsymbol{r}) \boldsymbol{b}_i = \boldsymbol{0} \quad  & \boldsymbol{b}_i^T \boldsymbol{M} \boldsymbol{b}_i = 1 \quad  \boldsymbol{b}_i^T \boldsymbol{M} \boldsymbol{b}_j = 0  \quad  \forall j \neq i 
\label{eq:gevp-with-locality-minimization}
\end{align}



We minimize the above energy using block coordinate descent.
\paragraph{Global Step}

\begin{align}
\argmin_{\boldsymbol{b}_i}\,&  \boldsymbol{b}_i^T \boldsymbol{H} \boldsymbol{b}_i \nonumber  \\  \text{s.t.} \quad \boldsymbol{b}_i^T {\boldsymbol{S}^{n-1}}  = \boldsymbol{0} \quad  & \boldsymbol{b}_i^T \boldsymbol{M} \boldsymbol{b}_i = 1 \quad  \boldsymbol{b}_i^T \boldsymbol{M} \boldsymbol{B} = 0  \nonumber
\end{align}

We can introduce $\boldsymbol{u}_i = \boldsymbol{C}^T\boldsymbol{b}_i$
\begin{align}
\argmin_{\boldsymbol{u}_i}\,&  \boldsymbol{u}_i^T \boldsymbol{C}^T \boldsymbol{H} \boldsymbol{C} \boldsymbol{u}_i \nonumber  \\  \text{s.t.} \quad   & \boldsymbol{u}_i^T \boldsymbol{C}^T \boldsymbol{M}\boldsymbol{C} \boldsymbol{u}_i = 1 \quad  \boldsymbol{u}_i^T \boldsymbol{C}^T \boldsymbol{M} \boldsymbol{B} = \boldsymbol{0}  \nonumber
\end{align}

Enforcing the linear equality constraint via lagrange multipliers:

\begin{align}
\argmin_{\boldsymbol{u}_i, \boldsymbol{\mu}_i}\,&  \boldsymbol{u}_i^T \boldsymbol{C}^T \boldsymbol{H} \boldsymbol{C} \boldsymbol{u}_i + \boldsymbol{u}_i^T \boldsymbol{C}^T \boldsymbol{M} \boldsymbol{B} \boldsymbol{\mu}_i \nonumber  \\  \text{s.t.} \quad   & \boldsymbol{u}_i^T \boldsymbol{C}^T \boldsymbol{M}\boldsymbol{C} \boldsymbol{u}_i = 1 \nonumber
\end{align}

Enforcing the quadratic constraint via Lagrange multipliers:

\begin{align}
\argmin_{\boldsymbol{u}_i, \boldsymbol{\mu}_i, \lambda_i},  \,&  \boldsymbol{u}_i^T \boldsymbol{C}^T \boldsymbol{H} \boldsymbol{C} \boldsymbol{u}_i + \boldsymbol{u}_i^T \boldsymbol{C}^T \boldsymbol{M} \boldsymbol{B} \boldsymbol{\mu}_i + \boldsymbol{u}_i^T (\boldsymbol{C}^T \boldsymbol{M}\boldsymbol{C} \boldsymbol{u}_i - 1) \lambda_i \nonumber 
\end{align}

Deriving the KKT optimality conditions:

\begin{align}
2 \boldsymbol{C}^T \boldsymbol{H} \boldsymbol{C} \boldsymbol{u}_i +  \boldsymbol{C}^T \boldsymbol{M} \boldsymbol{B} \boldsymbol{\mu}_i +  2\boldsymbol{C}^T \boldsymbol{M}\boldsymbol{C} \boldsymbol{u}_i \lambda_i 
 = \boldsymbol{0} \nonumber \\
 \boldsymbol{C}^T\boldsymbol{M}   \boldsymbol{B}  \boldsymbol{u}_i = \boldsymbol{0} \\
\boldsymbol{u}_i^T\boldsymbol{C}^T \boldsymbol{M}\boldsymbol{C} \boldsymbol{u}_i = 1
 \nonumber
 \end{align}
 
Which we can rewrite as the constrained GEVP:

\begin{align}
\begin{bmatrix}
\boldsymbol{C^THC} & \boldsymbol{C}^T\boldsymbol{M} \boldsymbol{B} \\
\boldsymbol{B}^T \boldsymbol{M} \boldsymbol{C} & \boldsymbol{0}
\end{bmatrix}
\begin{bmatrix}
\boldsymbol{u}_i  \\
\boldsymbol{\mu}_i  
\end{bmatrix} =
\lambda_i
\begin{bmatrix}
\boldsymbol{C}^T \boldsymbol{M} \boldsymbol{C} &
\boldsymbol{0} \\ \boldsymbol{0} & \boldsymbol{0}
\end{bmatrix}
\begin{bmatrix}
\boldsymbol{u}_i  \\
\boldsymbol{\mu}_i  
\end{bmatrix}
\end{align}

\paragraph{Local Step}

Starting from  Equation \ref{eq:gevp-with-locality-minimization}, we can enforce our locality constraint through Lagrange multipliers:
\begin{align}
\argmin_{ \boldsymbol{c}_i, \boldsymbol{\gamma}_i}\,&  \boldsymbol{b}_i^T \boldsymbol{H} \boldsymbol{b}_i + \boldsymbol{\gamma}^T_i \boldsymbol{S}(\boldsymbol{c}_i; \boldsymbol{r}) \boldsymbol{b}_i \\  \text{s.t.}  \quad  & \boldsymbol{b}_i^T \boldsymbol{M} \boldsymbol{b}_i = 1 \quad  \boldsymbol{b}_i^T \boldsymbol{M} \boldsymbol{b}_j = 0  \quad  \forall j \neq i 
\end{align}
We then omit all terms that do not depend on our center of locality $\boldsymbol{c}_i$
\begin{align}
\argmin_{ \boldsymbol{c}_i, \boldsymbol{\gamma}_i}\,&  \boldsymbol{\gamma}_i^T \boldsymbol{S}(\boldsymbol{c}_i; \boldsymbol{r}) \boldsymbol{b}_i 
\end{align}
The above optimization problem penalizes non-zero terms that exist outside of our region of locality $\boldsymbol{S}(\boldsymbol{c}_i, r)\boldsymbol{b}_i$.  This is equivalent to maximizing the number of  non-zero terms inside our region of locality.
\begin{align}
\argmax_{ \boldsymbol{c}_i}\,&  \boldsymbol{C}(\boldsymbol{c}_i; \boldsymbol{r}) \boldsymbol{b}_i 
\end{align}
We can leverage the fact that the only possible number of $\boldsymbol{c}_i$ is finite because our problem is discrete. We can find $\boldsymbol{c}_i$ in O(n) time with the right data structure.  \Otman{Get back to this, maybe will omit this section entirely based on the decision we come to}

==> old_method.tex <==

\subsection{Clustering}
% 
\alec{We should separate ``clustered elasticity'' (where we have a moderate contribution for $\nu > 0$) and ``how we make clusters'' (where we don't have much of a contribution and probably we could really improve things)}

We describe a general clustering-based approach to accommodate non-linear elastic energies $E(\boldsymbol{u}^c)$ and to maintain a mesh resolution independent simulation step. We start by presenting our approach very broadly, and show how to apply the methodology specifically to an ARAP elastic energy and a Co-Rotational elastic energy.

We assume an elastic energy that can be decomposed into the sum of a quadratic and a non-linear energy terms, $\Psi$ and $\Phi$ respectively, that are piece-wise constant over each tetrahedron $t \in \mathcal{T}$ in our mesh. 

\begin{equation}
    E(\boldsymbol{u}^c) = \underbrace{\sum_t^\mathcal{T} \Psi_t(\boldsymbol{u}^c)}_{quadratic} + \underbrace{\sum_t^\mathcal{T}  \Phi_t(\boldsymbol{u}^c)}_{non-linear}
\end{equation}

The sum over tetrahedra in the first term can be rewritten in simple matrix vector notation; a sum of quadratics is a quadratic as well. Starting with the general form of a quadratic energy for the first term and plugging in $\boldsymbol{u}^c = \boldsymbol{B} \boldsymbol z$ we can re-express this energy entirely in terms of reduced space operations.

\begin{equation}
\sum_t^\mathcal{T} \Psi_t(\boldsymbol{u}^c)  = \frac{1}{2} \boldsymbol{z}^T  \underbrace{\boldsymbol{B}^T \boldsymbol{\mathcal{H}} \boldsymbol{B}} \boldsymbol{z} + \underbrace{\boldsymbol{B}^T \boldsymbol{\mathcal{J}}^T}\boldsymbol z
\end{equation}

Where $\boldsymbol{\mathcal{H}}$  is a matrix of quadratic coefficients and $\boldsymbol{\mathcal{ J}}$ is a vector of linear coefficients. 

We focus now on the non-linear term, which in general is difficult to express in our reduced space basis. In particular, we can no longer simply rewrite this sum into a pre-computable system matrix $\boldsymbol{\mathcal{H}}$ like we did in the quadratic term. As a result, evaluation of this energy at run-time requires per-tet computation. To avoid this, we introduce a second set of acceleration parameters, tetrahedron \textit{clusters}. 

The intuition is that many tetrahedra will often exhibit similar energy profiles. In such cases we group these similar deforming tets into a \textit{cluster}. Then,  we only compute a single non-linear energy contribution term for each cluster, and simply use the same one for the other tetrahedra belonging to that cluster. Assuming we pick less clusters than there are tetrahedra, our speed-up is \textit{assured}. 


We now rewrite the second non-linear energy term in terms of per-cluster contributions. 

\begin{equation}
\sum_t^\mathcal{T} \Phi_t(\boldsymbol{u}^c)  \approx \sum_c^\mathcal{C} \Phi_c(\boldsymbol{u}^c)
\end{equation}

In order to rewrite our non-linear term as a function of our reduced space coefficients, we need to make one final assumption about the structure of our per-tetrahedron energy. We assume that the per-tetrahedron energy can be fully rewritten in terms of the per-tetrahedron deformation gradient $\Phi_{t}(\boldsymbol{u}^c) = \Phi_{t}(\boldsymbol{u}^c)  = \Phi_{t}(\boldsymbol{F}_t) $ $ \boldsymbol{F}_t \in \mathbb{R}^{ 3 \times 3}$. We can concatenate a list of flattened deformation gradients into a vector $\boldsymbol{\bar{F}} \in \mathbb{R}^{9t\times 1}$ and in turn express it as a simple linear function of our complementary displacement field $\boldsymbol{\bar{F}}  = \boldsymbol{K} \boldsymbol{u}^c + \boldsymbol{H}$ as derived in the Appendix \ref{section:Appendix}.
\Otman{We can relax and generalize this assumption (dependance on F) a bit more though.} 

We introduce the grouping matrix $\boldsymbol{G}_\Sigma \in \mathbb{R}^{\mathcal C \times \mathcal T}$, which sums contributions from individual tetrahedra over all clusters. Equipped with our grouping matrix, we approximate the second non-linear term:


%\begin{align*}
%\Psi (\boldsymbol{u}^c)  &= \frac{1}{2}{\boldsymbol{u}^c}^T \boldsymbol{\mathcal H} \boldsymbol{u}^c - \boldsymbol{\mathcal{J}}^T \boldsymbol{u}^c \\
%\Phi (\boldsymbol{u}^c) &= \frac{1}{2}
%\end{align*}



\subsubsection{Elastic Energy Gradient Evaluation}
Many elastic energies and their gradients rely on integrating per-tetrahedral strain quantities. To facilitate discussion, we assume a linear co-rotational elastic energy \cite{SifakisNotes}, but our clustering scheme could theoretically be used for any energy that is written as a function of per-tetrahedral deformation gradients. 

\begin{align}
E(\boldsymbol{u}^c) &= \int_\Omega \Psi(\boldsymbol F) d\Omega \\
&= \int_\Omega \frac{\mu}{2} ||\boldsymbol F - \boldsymbol R||^2_F +  \frac{\lambda}{2} ( tr(\boldsymbol R^T \boldsymbol F - \boldsymbol I))^2 d\Omega 
\end{align}

Where $\boldsymbol F \in \mathbb{R}^{3x3} = \frac{\partial \boldsymbol x}{\partial \boldsymbol X} = \frac{\partial \boldsymbol u^c}{\partial \boldsymbol X} + \frac{\partial \boldsymbol{u^r}}{\partial \boldsymbol X} + \boldsymbol I$ is the per tetrahedron deformation gradient, measuring how a deformed position $\boldsymbol x$ changes in each direction as we perturb our rest configuration. We assume linear elements, and as a result this deformation gradient is piecewise constant over each tetrahedron. $\boldsymbol R \in \mathbb{R}^{3 \times 3}$ is a per-tetrahedron rotation, obtained commonly via a polar decomposition of $\boldsymbol F$. The first term penalized shear and scaling deformations and the second term penalizes volume change, both done while remaining invariant to rotations. The Lamé parameters $\mu$ and $\lambda$ allows us to weigh these two elastic properties for our material. We're particularly interested in the gradient of this energy for each tetrahedron.

\begin{align}
\frac{\partial E(\boldsymbol{u}^c)}{\partial \boldsymbol{u}^c} &=  
\int_\Omega \frac{\partial \boldsymbol{F}}{\partial \boldsymbol u^c}^T \frac{\partial \Psi(\boldsymbol{F})}{\partial \boldsymbol{F}}  d\Omega\\
 &=\int_\Omega \frac{\partial \boldsymbol{F}}{\boldsymbol u^c}^T \underbrace{( \mu (\boldsymbol F  - \boldsymbol R) + \lambda tr(\boldsymbol R^T \boldsymbol F - \boldsymbol I)\boldsymbol R)}_{\boldsymbol{\Phi}}  d\Omega
\label{eq:gradient_corot_2}
\end{align} 

We denote the constant per-tetrahedron quantity $\frac{\partial \Psi(\boldsymbol{F})}{\partial \boldsymbol{F}}$ with $\boldsymbol \Phi$ for convenience.  We can efficiently compute all per-tetrahedra deformation gradients $\boldsymbol{F}$ from our displacements and reduced space coefficients through a simple matrix multiplication:
\begin{align}
    \boldsymbol{\bar{F}} &= \boldsymbol{K} \boldsymbol u^c + \boldsymbol{K} \boldsymbol u^r +  \boldsymbol{\bar{I}} \\
     &= \boldsymbol{K} \boldsymbol{B} \boldsymbol z + \boldsymbol{K} \boldsymbol u^r +  \boldsymbol{\bar{I}}
     \label{eq:full_deformation_gradient_from_reduced_coefficients}
\end{align}

Where we introduce $\boldsymbol{\bar{F}} \in \mathbb{R}^{9|T|}$ to denote a list of flattened deformation gradients. $\boldsymbol{\bar{I}} \in \mathbb R^{ 9|T|}$ is a  similar list of flattened identity matrices for each tetrahedron, and the sparse matrix $\boldsymbol{K} \in \mathbb{R}^{9|T| \times 3n}$ maps displacements to their contributions in the deformation gradient and is derived in the appendix \Otman{write this section in the appendix}. 
Splitting up Equation \ref{eq:gradient_corot_2} into the piecewise constant contributions from each tetrahedra, we can write a compact matrix expression to efficiently compute the discrete full space gradient $\boldsymbol{g}$.

\begin{align}
\boldsymbol{g} = \frac{\partial E(\boldsymbol{u}^c)}{\partial \boldsymbol{u}^c} =   \frac{\partial \boldsymbol{\bar{F}}}{\partial \boldsymbol u^c}^T  \boldsymbol{\mathcal{M}}\boldsymbol{\bar{\Phi}} = \boldsymbol{K}^T  \boldsymbol{\mathcal{M}}\boldsymbol{\bar{\Phi}}
\label{eq:discrete_gradient_corot}
\end{align} 

$\boldsymbol{\bar{\Phi}} \in \mathbb{R}^{9|T|}$ denotes another list of flattened per tetrahedra $\boldsymbol \Phi$ and $\boldsymbol{\mathcal{M}} \in \mathbb{R}^{9|T| \times 9|T|}$ is a diagonal matrix containing per-tetrahedra volumes. We now hold all the pieces required to compute the discrete energy gradient $\boldsymbol g$ from our reduced space coefficients $\boldsymbol z$. We first obtain the per tetrahedron deformation gradient $\boldsymbol{\bar{F}}$ using Equation \ref{eq:full_deformation_gradient_from_reduced_coefficients}. Then, for each tetrahedron we perform a polar decomposition on its deformation gradient $\boldsymbol F$ to achieve a corresponding best-fit rotation $\boldsymbol R$. Using these two per-tet quantities, we evaluate a list of $\boldsymbol Phi$, flatten them and stack them into them into $\boldsymbol{\bar{\Phi}}$. Finally, we use Equation \ref{eq:discrete_gradient_corot} to evaluate our final gradient.

While this current approach still has many steps that can be precomputed away, it will ultimately always require the computation of per tetrahedra quantities in $\boldsymbol{\bar{\Phi}}$. Unfortunately, our mesh may have a large number of tetrahedra, preventing even our reduced model from achieving interactive rates as shown in Figure \ref{fig:reduction-time-complexity}. 

\subsubsection{Clustering Methodology}
\alec{This section is way too long. Should be a paragraph.}
We prevent the gradient evaluation from scaling in time with the number of tetrahedra by making use of clustering, with the intuition that tetrahedra exhibiting similar motion could be reasonably approximated to have the same deformation gradient. This would allow us to only have to evaluate a single value of $\boldsymbol{\Phi}$ per \textit{cluster}, where we would obtain a performance boost when the number of clusters is smaller than the number of tetrahedra. 

\begin{wrapfigure}{r}{3.0cm}
\includegraphics[width=\linewidth]{images/cactus-clusters}
\caption{Clusters for the 2D cactus in Fig.~\ref{fig:cactus-modes}.}
\end{wrapfigure}
%
We make use of the very standard kmeans++ \cite{kmeanspp} clustering algorithm, grouping tets with similar features together. As input to this routine, we provide a set of per-tetrahedral features. 
We desire to delegate more clusters to regions of our mesh that will exhibit a lot of secondary motion, and less in regions that show very little motion. Our reduced subspace $\boldsymbol B$ encodes \textit{exactly} that sort of information! Each of its columns represents an energetically favourable deformations that satisfies complementarity. Even better, the columns are already sorted sorted in order of how favourable they are. As a result we make use of our constrained, reduced subspace $\boldsymbol B$ to build our tetrahedral features.

For each tetrahedron, we slice out the rows of $\boldsymbol B$ that belong to the four vertex indices incident on our tetrahedron; there will be 12, seeing as each vertex actually owns 3 rows (one for each of the 3D axes $\{x, y, z\}$). We concatenate the 3 rows for each vertex, then take take the mean over the remaining 4 rows and end up with a single feature vector $f \in \mathbb{R}^3m$.

We take note of \citet{Lipman:2010:BD} and follow the intuition that smaller magnitude modes should contribute more deformation information than high magnitude modes. As a result we divide each modal feature in our subspace vector by it's corresponding eigenvalue. We also find that as a result we get quickly diminishing returns on the number of modes we need to use to build our features, and obtain a very reasonable cluster set with only the first 5 modes as shown in Figure \ref{fig:diminishing_modal_returns}.

\begin{figure}
\includegraphics[width=\linewidth,keepaspectratio]{images/white.png}
\caption{\Otman{Our clusters using 1 mode, vs, 5 modes, vs 10, vs 100, while also showing how long it took to build them}}
\label{fig:diminishing_modal_returns}
\end{figure}

We compare our subspace features to using Euclidean features, and to using weight-space features as in \citet{Jacobson-12-FAST} in Figure \ref{fig:clustering-features}. Our features results in clusters that are both rig aware and dynamics aware, correctly shying away from regions more heavily influenced by the rig, while also more densely populating regions that are likely to experience secondary motion.

Our kmeans++ routine will output a list of cluster labels, which we can use to build an averaging grouping matrix $\boldsymbol{G}_w \in \mathbb R^{ 9|c| \times 9 |T|}$, which performs a mass weighted averaging of the deformation gradient for each tet in a given cluster. Using this matrix, and our formula for obtaining the deformation gradient of each tet from our displacement, we obtain an efficient way of obtaining this weighted clustered deformation gradient. \Otman{See section in Appendix, which needs to be written}.

\begin{align}
    \boldsymbol{\bar{F}}_{c} = \boldsymbol{G}_w \boldsymbol{\bar{F}} =  \underbrace{\boldsymbol{G}_w\boldsymbol{K} \boldsymbol{B}}_{\boldsymbol H} \boldsymbol{z} + \underbrace{\boldsymbol{K} \boldsymbol{u}^r}_{\boldsymbol {\bar{d}}} + \boldsymbol{\bar{I}}
    \label{eq:clustered_defo_gradient}
\end{align}

Where we introduce $\boldsymbol{\bar{F}} \in \mathbb R^{ 9|T|}$ our list of flattened deformation gradients for each tet, and $\boldsymbol{\bar{{F}}_c} \in \mathbb R^{ 9|c|}$, the same list but for each cluster. $\boldsymbol{H} \in \mathbb{R}^{9|c|\times m}$ is a dense matrix that can be precomputed at the start of the simulation, and $\boldsymbol{\bar{d}} \in \mathbb{R}^{9|c|}$ at the start of each timestep as soon as the rig motion is known.

Once we have our per-cluster deformation gradient, we can easily construct a list of concatenated $\boldsymbol{\bar{\Phi}}_c$. We can then obtain our full space gradient through a slight modification of Equation \ref{eq:discrete_gradient_corot}:

\begin{align}
\boldsymbol{g} = \frac{\partial E(\boldsymbol{u}^c)}{\partial \boldsymbol{u}^c}  = \boldsymbol{K}^T  \boldsymbol{G}_1^T\boldsymbol{\mathcal{M}_c}\boldsymbol{\bar{\Phi}_c}
\label{eq:discrete_gradient_corot_clustered}
\end{align} 
 
 Where we make use of our grouping matrix  $\boldsymbol{G}_1 \in \mathbb R^{ 9|c| \times 9 |T|}$ that sums across tets in each cluster, and $\boldsymbol{\mathcal{M}} \in \mathbb{R}^{9c \times 9c}$ is a diagonal matrix with per-cluster volumes. % Equation \ref{eq:reduced_solve} specifically involves projecting this gradient into our reduced subspace,

\subsubsection{Cluster-induced Null Space}

Running the clustering scheme above with a full simulation can lead to disastrous results, as seen in Figure \ref{fig:null_space_vis}. The clustering seems like it introduces a source of plasticity into the simulation. This is actually because of a null-space that expresses itself in our optimization as plasticity. This occurs because multiple configurations of tetrahedra in our cluster can average out to measure the same deformation gradient. Figure \ref{fig:null_space_vis} shows a didactic example showing a rest configuration with an identity deformation gradient for the cluster, and a deformed configuration that also measures an identity-valued clustered deformation gradient.

We can show the existence of this null-space mathematically by looking at our expression for our clustered deformation gradient in Equation \ref{eq:clustered_defo_gradient}. Each of the 9 entries $ij$ for each of our deformation gradients is uniquely obtained by slicing out the blocks of our matrix multiplication in \ref{eq:clustered_defo_gradient}, $(\boldsymbol{G}_w \boldsymbol K)_{ij} \in \mathbb{R}^{c \times |T|}$.

\begin{align}
    \boldsymbol{\bar{F}_c}_{ij} = (\boldsymbol{G}_w \boldsymbol K)_{ij} \boldsymbol{u^c} + \boldsymbol C 
    \label{eq:null-space-deformation-gradient}
\end{align}
$\boldsymbol{C}$ is a placeholder term absorbing all terms that do not depend on $\boldsymbol u^c$ in Equation \ref{eq:clustered_defo_gradient}. The matrix mapping from our displacements to our deformation gradient entries is a rectangular, undetermined one. In other words, it shows mathematically what we discussed earlier, that there exists multiple solutions that map to the same deformation gradient. All it takes in order to avoid this null-space is for the number of clusters to be equal to the number of degrees of freedom, so that this mapping matrix becomes square. Thankfully, our model reduction based algorithm lets gives us free reign in choosing how many degrees of freedom we want our simulation to have, and so our system can easily sidestep this issue, while maintaining freedom in our choice of modes and cluster configurations.



\begin{figure}
\includegraphics[width=\linewidth,keepaspectratio]{rough_images/null_space_clustering.jpg}
\caption{Our clustering scheme introduces a null space, which allow non-rest states to erroneously measure zero energy, and introduces artificial plasticity into our simulation. \Otman{Show the plasticity introduction}}
\label{fig:null_space_vis}
\end{figure}


\begin{figure}
\includegraphics[width=\linewidth,keepaspectratio]{rough_images/clustering-scheme.jpg}
\caption{Clustering an elephant mesh, controlled by a single handle rig (need to show this) with Euclidean space features, weight-space features \cite{Jacobson-12-FAST} and our constrained subspace features. Euclidean features(left) group tets like the trunk and the belly, that are close together in euclidean space but far away semantically. Weight space features (middle) cluster vertices that are controlled by the rig in a similar fashion similarly, because this is a single point affine rig, all vertices share the exact same weight value and so clusters are formed randomly accross the mesh.
Our clustering in B-space groups together semantically intuitive features, vertices that move together in the space of motions irreproducible by the rig.} 
\Otman{Show another example using a LBS rig}
\label{fig:clustering-features}
\end{figure}



\begin{figure}
\includegraphics[width=\linewidth,keepaspectratio]{rough_images/clustering_incompressibility.jpg}
\caption{Our clustering scheme applied to a standard co-rotational elasticity model (no model reduction applied to this example). We obtain substantial speedups while still reproducing key incompressible deformations.}
\label{fig:clustering-corotational}
\end{figure}

\begin{figure}
\includegraphics[width=\linewidth,keepaspectratio]{rough_images/clusters_timing.jpg}
\caption{An analysis of how our run-time varies with the number of clusters on different meshes. Our method depends linearly on the number of clusters.}
\label{fig:clustering-time-complexity}
\end{figure}



\begin{figure}
\includegraphics[width=\linewidth,keepaspectratio]{rough_images/pareto-front.jpg}
\label{fig:clustering-time-complexity}
\caption{An analysis of an empirically obtained pareto-front, showing optimal num modes/ numclusters required to obtain real-time (24FPS) modes.}
\end{figure}


%These clusters would better be spent on augmenting the motion around the trunk and rigs, as they correctly are identified with our rig-constrained subspace features (right).}
%Tetrahedra in the torso are clustered together, when in fact they will undergo very little motion. 


==> old_related.tex <==

\section{Related Work}
Solving for elastodynamics usually involves having to construct a large sparse system of equations, and then solving it each timestep. Accelerating elastodynamics has been a primary point of interest in graphics since the the pioneering work of \cite{Terzopoulos1987}. 

The most obvious way of speeding up this system solve is by using a fast linear solver. Because the system usually changes each timestep, direct solvers making use of matrix pre-factorizations are off the table. Iterative solvers, such as Conjugate Gradient, LBFGS or multigrid solvers \cite{LiuMultigrid2021} find a solution in time complexity \emph{linear} with the mesh resolution. 

Aside from selecting an optimal linear solver, we can also reformulate the discretization of the underlying physics.
Position based dynamics 
\cite{MullerPBD2007, MullerMeshlessDefo2005, MacklinPBDStableNeohookean2021} model  elasticity using only point masses and a set of elasticity-enforcing constraints. The point masses are integrated in time with a forward euler integration step, after which their positions are projected to an elasticity-inspired constraint manifold. This process is repeated until satisfaction. The resulting dynamics are tied to the number of iterations/constraint projection steps are performed, where each iteration scales linearly in complexity with the number of points and constraint projection steps.

\paragraph{Projective Dynamics}
\cite{Bouaziz:2014:Projective} formalizes the process above by identifying exactly a class of elastic energies that can be described by a non-linear constraint projection step, and a standard linear solver. Specifically, these energies satisfy that the constraint projection step handles all of the complex changing non-linear behavior, leaving the resulting system static. The static system allows us to prefactorize the system. 
\cite{QuasiNewtonLiu2017}  and \cite{Narain2016} generalize projective dynamics to a broader class of elastic materials by linking it to broader optimization schemes, like ADMM and Quasi-Newton Methods.
Iteratively solving for the constraints and the degrees of freedom can cause slow convergence, \cite{MixedFEMTrusty2022} greatly accelerate the convergence through a Mixed Finite Element scheme, essentially linking the constraints to the degrees of freedom with lagrange multipliers to make sure the two are always in agreement. 



 Boundary element methods \cite{Sugimoto:2022:BEM, artDefoJames1999} for elasticity require dense solves and a complicated implementation overhead to obtain linear-time advertised speedups.


\cite{McAdams2011} provide a grid-discretized cubtature accelerated elasticity model.

\subsection{Reduced Models for Elasticity}


\paragraph{Linear  Subspaces from Modal Analysis} Subspaces obtained via modal analysis have been used in graphics since \citet{PentlandWilliams1989} as a way to accelerate physics-simulations. Instead of obtaining the linear basis from a statistical basis, they obtain it through a modal analysis of the elastic energy. Here, the subspace is spanned by the lowest-energy deformations as computed from the rest state of the system, which end up being the eigenvectors of the rest state elastic energy Hessian. The resulting physical simulation is then performed in the subspace, where the simulator aims to find how much to activate each of these low-energy vectors. The  resulting motions suffer from linearization artefacts, and are not rotation equivariant. \cite{BarbicJames:RealTimeSTVK}.  

\cite{HarmonSubspaceLocalDeformation2013} and \cite{Teng:SubspaceCondensation} add local enrichment functions on the fly.
\cite{melzi2018localized} compute local modes with a weighing parameter in a least squares sense. 
\cite{compressedModesADMM}  and \cite{Brandt2017CompressedVibrationModesofElasticBodies} compute modes with a sparsity penalizing $l_1$ regularization term and minimizing the resulting energy with ICCM or ADMM respectively. This sparsity term is balanced by the smoothness measured by the elastic energy hessian creates modes that are \emph{local}. This results in a slow process that requires a lot of tweaking of parameters, and the delicate balance between the smoothness and the sparsity term can easily be corrupted with additional constraints in the optimization.


\paragraph{Augmenting Subspaces with Modal Derivatives}
A big drawback of linear subspaces is just that, their \emph{linearity}. As a subspace simulation is excited and undergoes large deformation (deviating from the rest state), the set of basis vectors spanning our subspace quickly becomes sub-optimal. Modal derivatives \cite{BarbicJames:RealTimeSTVK} augment these linear bases with a new set of \emph{derivative} modes, whose aim is to provide the support needed for the simulation to update the primary set of modes in order to better acommodate the large deformation. These modes effectively make the subspace a \emph{quadratic} one instead of a linear one.  While the quality of subspace simulations making use of modal derivatives is greatly increased,  this is a band aid. Modal derivatives struggle to reproduce even simple global rotations as shown in Figure \ref{fig:subspace-comparisons}.  
\paragraph{Modal Warping}
\alec{What do you mean by ``floating frame''? How is that different from a ``frame''? There a bunch of ``frame-based'' methods (see Benjamin Gilles and Francois Faure) methods that we should distinguish ourselves from.} \Otman{ah good point... i consider Gilles and Faures methods to be a skinning subspaces for deformation. we definitely should distinguish our method from theirs in that section. what I mean here by floating frame is just updating the displacement modes each timestep with a best fit rotation matrix.}
\citet{ModalWarping} Computes a best-fit rotation matrix at each vertex, and updates each vertex's subspace with that corresponding rotation. While this allows the subspace simulation to accommodate local rotations and maintain rotation equivariance, the process of updating the subspace is a full space operation. This method quickly become prohibitively expensive for large meshes. 

\paragraph{Sub-structuring}
We can instead identify sub-structures in our mesh that should exhibit similar rotational properties, either specified by a user \cite{Barbic:2011:RealTimeLargeDefoSubstructuring}, or automatically detected via a clustering-like approach \cite{KimJamesMultiDomainStitching}.The subspace is then updated on a per-region basis (instead of per-vertex like Modal Warping). Too few sub-structures means our subspace loses out on representing local rotational motion. More sub-structures allow for the capture of rotational deformations, but requires updating the subspace for each sub-structure; an operation that becomes the bottleneck in our subspace simulation, limiting the richness of the dynamics we can obtain at real-time speeds. Additionally, to perform this subspace update quickly, one would use a Fast Sandwich Transform \citet{FST}, which requires a heavy memory budget at the pre-computation stage (Each substructure requires precomputing any matrix involving the subspace 9 times, 1 for each rotation parameter). 

\paragraph{Rotation Strain Coordinates}
Rotation strain coordinates take linearized deformations and project them to a best-fit rotational motion via an exponential map. Ironically, that deformation \emph{needs} to be linearized... if the deformation were a simple non-linear global rotation, it is prone to catastrophic collapse. To avoid this you need to use a floating frame, or many floating frames, for which we discuss disadvantages above. Additionally, enforcing the complementary constraint in this rotation-strain coordinate system is not immediately obvious, where should we enforce it? On our simulation step, or on the projection step? On both?

\paragraph{Skinning Subspaces}
Using linear blend skinning as a deformation subspace is not new. All prior methods differ in how they construct their linear blend skinning subspace.
\citet{RSPHahn} let's a user specify their own physics-rig and develop a physical simulation that acts on that rig-space specifically.  This burdens the user with specifying their own rig and rig-weights an often unintuitive task. A user may easily be able to specify low frequency physical motions they may want in their subspace, but it's often harder for them to think of the fine detail.  Our method assumes a linear blend skinning subspace for secondary motion, and we build an optimal secondary linear blend skinning subspace automatically from the primary control rig, unburdening this task user. 
\citet{Brandt2018HyperReducedPD} build their linear blend skinning subspace weights very quickly via normalized radial basis functions. While this method is very fast and effective, it unfortunately is not material aware. Resulting in inefficient simulations. 
\citet{Gilles2011} compute a material aware \emph{Dual Quaternion Skinning} subspace (as opposed to a skinning subspace) for deformation. They require a user to specify as input \emph{frames}, and then from those frames they construct weight functions using harmonic coordinates \cite{Joshi2007}.  While these weights are smooth and localized around each frame, they are not material aware.
\citet{Faure2011} improve upon the above, and specifically automatically determine where to place the initial input frames, and compute weights proportional to a material-aware quantity: \emph{the compliance distance}. 


All three of the above cannot accommodate the complementary constraint.

\paragraph{Cubature}
To accommodate rotational deformations, elastic energies require the use of per-tet non-linear energetic quantities. As a result, even with the use of a subspace approximation on our degrees of freedom, our simulation  complexity is still tied to the resolution the meshes in question. To remedy this \citet{OptimizingCubature} make use of a \emph{cubature} integration scheme, approximating these per-tet non-linearities with a sparse set of carefully chosen sample tetrahedra. These non-linearities are then computed on this smaller set of tetrahedra, which are blended with cubature weights to recuperate the per-tetrahedral non-linearities. 

This approach's success is heavily dependant on the selection of the sample tetrahedra. These samples are often found by a least squares fitting to some training data. A poor sample set can result in obvious deformations not in the training data to go completely ignored. We instead make use of clusters, which are not constructed from training data, but rather an elasticity prior.

\paragraph{Clustering}
Addressing the same issue as above \cite{Jacobson-12-FAST} make use of non-linearity \emph{clusters}. Instead of approximating these non-lineariteis with a sparse set of samples, clustering groups tetrahedra together and performs a weighed average on these non-linear quantities. 
As a result, any deformation occurring at any tetrahedra can still be represented and felt. Their use case applies clustering only to an ARAP elastic energy, whereas we show we can apply this clustering methodology to a much larger set of elastic energies. 



\paragraph{Neural Elastodynamic Simulation}
While recent approaches like \cite{zheng2021deep} show promise in being capable of learning efficient encoding for physical simulation, they still suffer from a number of difficulties. They require tons of training data. Their capacity to generalize across meshes has yet to be battle tested. While simulating a normal elastic material is a current open research problem, a neural simulator capable of outputting motions that satisfy the control constraint of complementary dynamics is still a while away. 



==> results_old.tex <==


\Otman{talk about global support of modes? Maybe that's not desireable? Need to change this once I experiment with local support}


\section {Results}
Our method specializes in applications that require dynamically changing control of high-resolution, elastic materials with complex rigs. We show real-time results for augmenting AR based skeleton-tracking with secondary motion, and discuss how our method could easily be incorporated into a character controller in a game engine.      


\subsection{AR Manipulation of Various Rigs}
We show that our approach can be used on any arbitrary rig, so long as we can define its rig Jacobian. We show a user controlling a wide range of geometry and rig combinations in Figure \ref{fig:ARDifferentRigs}. Fast Complementary Dynamics allows for a user to creatively explore how they wish to best interact with their scene. Note that some rigs control motion that is not trivially obtainable from physical simulation, such as the twisting motion obtained by QBS. \Otman{I want a really exotic rig, something like PSD}
\begin{figure}
\includegraphics[width=2cm,height=3cm,keepaspectratio]{images/white.png}
\caption{User controlling a Linear Blend Skinning rig, mapping their arms to the wings (left). User controlling a point handle rig, animating a walking velociraptor with their hand (middle). User controlling 4 seperate bones of a 4-legged monster with their legs and arms (right). User controlling a tall giraffe, twisting the giraffe's neck with a dual quaternion skinning rig.}
\label{fig:ARDifferentRigs}
\end{figure}


\subsection{Skeleton Tracking Affine Rig}
We use our method to augment rig motion obtained from a real-time skeleton pose-tracker. We make use of a publically available set of Deep Learning based tools in Mediapipe \cite{lugaresi2019mediapipe}, that capture a video live stream and outputs any detected skeletal joint positions in screen space and in world space. 

Figure \ref{fig:ARAffineRigElepehantDemo} shows a user manipulating an elephant with an affine rig. The user makes us all the rig's degrees of freedom, translating and rotating the elephant. This rig motion is given as input to our method and we obtain intuitive secondary motion, such as the trunk and ears moving around.

In comparison we show a similar framework, where a user controls the affine motion that is then a constraint on central vertices of the elephant. Notice that as the use moves the elephant around, we can clearly see undesired artifacts, anchoring the rest of the elephant around its seemingly steel center. 

\begin{figure}
\includegraphics[width=\linewidth, keepaspectratio]{rough_images/octopus_pinned_vs_cd.jpg}
\caption{A user controlling octopus tentacles with their hand through a live video stream hand tracker. We enforce rig-control through constraining vertices lying within the skeleton "bones" (top) and our real-time complementary dynamics with reduced subspace degrees of freedom and deformation gradient clustering(bottom). Real-time complementary dynamics naturally lets the tentacles wiggle and move freely, while directly enforcing vertex positions robs the simulation of rich secondary dynamics and leads to an overly stiff animation.}
\label{fig:octopus_pinned_cd_comparison}
\end{figure}


\begin{figure*}
\includegraphics[width=\textwidth]{images/pinned_vs_cd_fig.pdf}
\caption{
\alec{The left most figure confuses the setup. The reader has never seen the rest state of the octopus so they will assume that it's this image. I'd show the rig in its rest state and rely on the video timestamp (where are these?) to point readers to see the rig motion.}
Pinning vertices to enforce control over a simulation leads to strong visual artefacts, and a simulation that is difficult to control. Carefully choosing which vertices to pin is a burdensome experience for a user. Instead, enforcing control through our rig-complementary modes results in smooth and controllable behavior, staying faithful to the input rig motion while adapting it to a dynamic simulation.
\alec{Our deformation still exhibits some ``kinks'' at the tips. How come?}
}
\label{fig:octopus_pinned_cd_comparison}
\end{figure*}



\subsection{Fast CD vs Coarse Mesh CD}
We compare our fast Complementary Dynamics to simply results obtained from coarsening our mesh. Figure  that for the same computational budget, we can obtain much more rich deformation. 
We stress test our method directly on large tetrahedral meshes (500k vertices, 1.5 million tets). We show that we can maintain interactive frame rates for such high quality meshes. 

\begin{figure}
\includegraphics[width=\linewidth,keepaspectratio]{images/coarse_vs_reduced_fig.pdf}
\caption{
\alec{Try to eliminate any wasted white space. Think about the figure layout \emph{before} collecting the raw footage. This model is very tall, so it's harder to achieve a good horizontal layout. Maybe add another frame to make the figure 4-across with the cage inset.}
Reduced animation (50 modes, 50 clusters), vs full complementary dynamics on a coarser mesh.  Both take the same amount of time, but coarsening the mesh destroys so much animation detail. Look at the tongue on the velociraptor mesh and see how a coarse mesh groups the tongue with the rest of the mouth, same with the small arms and the torso, but our method lets the tongue be separate and free moving}
\label{fig:CoarseComparison}
\end{figure}

\begin{figure}
\includegraphics[width=\linewidth,keepaspectratio]{images/rig_space_physics_fig.pdf}
\caption{
\alec{white space again. For digaonally angled models you can even nest them a bit. This'll work even better if they're a bit more horizontally diagonal.
}
\alec{don't forget to add timestamps for all of these.}
}
\label{fig:RSPComparison}
\end{figure}

\subsection{Constrained Modes vs Unconstrained Modes}
We evaluate the effectiveness of using our modes, inherently satisfying the complementary constraint versus using unconstrained modes and enforcing the complementary constraint at run-time via lagrange multipliers.


\subsection{Augmenting Rigid Body motion}
Interactive rigid body simulations are commonly used in video games. We can augment such rigid body simulators with our pipeline with soft body wiggles, much like in \cite{Zhang:CompDynamics:2020}.
\Otman{bonus}
\section{Conclusion}
\Otman{Not done}

\section{Limitations}
\Otman{Express ingredients of our method :
Hessian at rest state
gradient evaluation of energy
energy expressed as a sum over elements that is a function of F
}
\Otman{Talk about nonlinear subspaces}

\Otman{Talk about clustering on different energies}

\Otman{Talk about exotic deep learning energies, finding deformation gradient}

\Otman{Clustering for different distributions of deformation spaces (bimodal multimodal ones)}

\Otman{ UV-mapping/parameterizations: use gradients to flatten}

\Otman{Deep learning : use gradients to perturb examples}

\Otman{ We're basically making a very weird look-up tables}

\Otman{ Our method : deformations obtained from rest-state features}

\Otman{Recursively subdivide pre-existing clusters for faster clusters}

\Otman{Help the user find the clusters}

\Otman{Rigid Body simulation}

\Otman{ How can we transform pre-computed parameters from one shape to a closely related shape}

\Otman{Eigen decomposition timings}
\Otman{Re-use precomputed modes to 
warm-start modal decomposition}
